Multi-Label Contrastive Learning : A Comprehensive Study

Multi-label classification, which involves assigning multiple labels to a single input, has emerged as a key area in both research and industry due to its wide-ranging applications. Designing effective loss functions is crucial for optimizing deep neural networks for this task, as they significantly influence model performance and efficiency. Traditional loss functions, which often maximize likelihood under the assumption of label independence, may struggle to capture complex label relationships. Recent research has turned to supervised contrastive learning, a method that aims to create a structured representation space by bringing similar instances closer together and pushing dissimilar ones apart. Although contrastive learning offers a promising approach, applying it to multi-label classification presents unique challenges, particularly in managing label interactions and data structure. In this paper, we conduct an in-depth study of contrastive learning loss for multi-label classification across diverse settings. These include datasets with both small and large numbers of labels, datasets with varying amounts of training data, and applications in both computer vision and natural language processing. Our empirical results indicate that the promising outcomes of contrastive learning are attributable not only to the consideration of label interactions but also to the robust optimization scheme of the contrastive loss. Furthermore, while the supervised contrastive loss function faces challenges with datasets containing a small number of labels and ranking-based metrics, it demonstrates excellent performance, particularly in terms of Macro-F1, on datasets with a large number of labels.

==> latex/0Abstract.tex <==
Multi-label classification, which assigns several labels to a single input, is central to many applications in computer vision and natural language processing. The loss function plays a decisive role in training deep networks for this task, yet conventional losses maximize a likelihood under a label-independence assumption and therefore struggle to capture complex label relationships. Supervised contrastive learning, which structures the representation space by pulling similar instances together and pushing dissimilar ones apart, offers a promising alternative, but its extension to the multi-label setting raises specific difficulties related to the definition of positive pairs, label interactions, and long-tailed label distributions. In this paper, we present a comprehensive study of contrastive losses for multi-label classification across diverse settings: datasets with small and large label spaces, full and limited training data, and both vision and text modalities. Our results show that the gains of contrastive learning stem not only from modeling label interactions but also from the favorable optimization behavior of the contrastive objective. We further identify its limitations: supervised contrastive losses are less effective on datasets with few labels and on ranking-based metrics, whereas they excel, particularly in Macro-F1, on datasets with many labels. Finally, building on a gradient analysis of the multi-label contrastive loss, we propose a regularized loss that cancels the gradient components that cause positive pairs to repel each other. The resulting loss is competitive with or outperforms existing contrastive and non-contrastive losses, with the largest gains in Macro-F1 and in low-data regimes.


==> table/dataset-semeval.tex <==
\begin{table}[t!]
\begin{center}
\caption{Statistics of the SemEval-2018 dataset: number of examples (in thousands) in the training, validation, and test sets, number of labels $L$, and average number of labels per example $\overline{L}$.}
\label{table:datasets}
%\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccc}
\toprule[1pt] % Makes the top line thicker
Dataset & $|\text{Train}|$ & $|\text{Val}|$ & $|\text{Test}|$  & L & $\overline{L}$ \\
\midrule
SEMEVAL & 6.6k & 1.k & 3.2k & 11 & 2.4 \\
\hline
\end{tabular}
\label{semeval:dataset}
\end{center}
\end{table}

==> table/nlp_small.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\small
\begin{tabular}{lccc ccc ccc}
\toprule[1pt] % Thick top rule
\multicolumn{1}{l}{} & \multicolumn{3}{c}{AAPD} & \multicolumn{3}{c}{RCV1} & \multicolumn{3}{c}{BGC} \\
\cmidrule(r){2-4} \cmidrule(lr){5-7} \cmidrule(l){8-10}
\multicolumn{1}{l}{\textbf{Loss}} & $\mu$-F$_1$ & M-F$_1$ & Ham & $\mu$-F$_1$ & M-F$_1$ & Ham & $\mu$-F$_1$ & M-F$_1$ & Ham \\
\cmidrule{1-10}
\multicolumn{10}{c}{\textbf{Non-Contrastive Losses}} \\
\cmidrule{1-10}
$\mathcal{L}_{BCE}$ & 68.76 & 49.49 & 25.93 & 86.90 & 70.39 & 93.10 & 74.28 & 49.61 & 100.58\\
$\mathcal{L}_{ASY}$ & 68.85 & 51.40 & 27.22 & 86.91 & 72.34 & 90.54 & 74.64 & 52.29 & 103.35\\
$\mathcal{L}_{ZLPR}$ & \textbf{69.45} & 50.98 & \textbf{25.69} & \textbf{87.39} & 72.05 & \textbf{88.20} & 75.49 & 53.22 & 98.37\\


\cmidrule{1-10}
\multicolumn{10}{c}{\textbf{Contrastive Losses}} \\
\cmidrule{1-10}
$\mathcal{L}_{Base}$ & 69.42 & 49.85 & 26.13. & 86.62 & 71.03 & 95.28 & 75.26 & 51.75 & 9.865\\
$\mathcal{L}_{Proto}$ & 69.09 & 51.05 & 27.79 & 86.52 & 72.91 & 97.59  & 74.82 & 53.38 & 10.52\\
$\mathcal{L}_{MulSupCon}$ & \textbf{69.39} & 49.01 & \textbf{25.70} & 86.96 & 71.84 & 93.00 & \textbf{75.57} & 51.93 & \textbf{97.74}\\
$\mathcal{L}_{MSC}$ & \textbf{69.45} & 50.69 & 26.77 & 86.91 & 72.49 &  94.16 & \textbf{75.63} & 52.57 & \textbf{97.69}\\
$\mathcal{L}_{W-REG}$ & 69.23 & 49.95 & 26.41 & 86.77 & 72.17 &  94.46 & 75.51 & 52.82 & 98.91\\
$\mathcal{L}_{REG}$ & 68.89 & \textbf{52.30} & 29.11 & 86.5 & \textbf{73.09} &  97.77 & 75.21 & \textbf{53.44} & 10.35\\

\bottomrule[1pt] % Thick bottom rule
\end{tabular}%
}
\vspace{2px}
\caption{20\% dataset : Comparative Analysis of multi-label loss functions on VOC, COCO, and NUS-WIDE datasets. Metrics used are Micro-F1 ($\mu$-F$_1$), Macro-F1 (M-F$_1$), and Hamming Loss (multiplied by $10^3$). The best results are highlighted in bold, including those that are not significantly different from the top-performing scores.}
\label{table:contrastive_losses}
\end{table*}


==> table/semeval.tex <==
\begin{table}[]
\centering
\caption{Comparison of multi-label loss functions on SemEval-2018. Metrics are Micro-F1 ($\mu$-F$_1$), Macro-F1 (M-F$_1$), and Hamming loss ($\times 10^3$). The best results, and those not significantly different from them, are in bold.}
\small
\begin{tabular}{lccc}
\toprule[1pt] % Thick top rule
\multicolumn{1}{l}{} & \multicolumn{3}{c}{SemEval} \\
\cmidrule(r){2-4}
\multicolumn{1}{l}{\textbf{Loss}} & $\mu$-F$_1$ & M-F$_1$ & Ham \\
\cmidrule{1-4}
\multicolumn{4}{c}{\textbf{Non-Contrastive Losses}} \\
\cmidrule{1-4}
$\mathcal{L}_{BCE}$ & 71.94 & 55.71 & \textbf{11.75} \\
$\mathcal{L}_{ASY}$ & \textbf{72.43} & \textbf{57.68} & 11.95\\
$\mathcal{L}_{ZLPR}$ & 71.52 & 55.7 & \textbf{11.76}\\

\cmidrule{1-4}
\multicolumn{4}{c}{\textbf{Contrastive Losses}} \\
\cmidrule{1-4}
$\mathcal{L}_{Base}$ & 70.91 & 57.60 & 12.68 \\
$\mathcal{L}_{Proto}$ & 69.99 & 56.08 & 12.89 \\
$\mathcal{L}_{MulSupCon}$ & 70.83 & 57.06 & 12.67\\
$\mathcal{L}_{MSC}$ & 69.98 & 56.19 & 12.98 \\
$\lwreg$ & 70.50 & 56.90 & 12.69 \\
$\lreg$ & 71.45 & \textbf{57.71} & 12.60 \\

\bottomrule[1pt] % Thick bottom rule
\end{tabular}%
\vspace{2px}
\label{table:contrastive-sem}
\end{table}

